Accoustate: Auto-annotation of IMU-generated Activity Signatures under Smart Infrastructure

Human activities within smart infrastructures generate a vast amount of IMU data from the wearables worn by individuals. Many existing studies rely on such sensory data for human activity recognition (HAR); however, one of the major bottlenecks is their reliance on pre-annotated or labeled data. Manual human-driven annotations are neither scalable nor efficient, whereas existing auto-annotation techniques heavily depend on video signatures. Still, video-based auto-annotation needs high computation resources and has privacy concerns when the data from a personal space, like a smart-home, is transferred to the cloud. This paper exploits the acoustic signatures generated from human activities to label the wearables' IMU data at the edge, thus mitigating resource requirement and data privacy concerns. We utilize acoustic-based pre-trained HAR models for cross-modal labeling of the IMU data even when two individuals perform simultaneous but different activities under the same environmental context. We observe that non-overlapping acoustic gaps exist with a high probability during the simultaneous activities performed by two individuals in the environment's acoustic context, which helps us resolve the overlapping activity signatures to label them individually. A principled evaluation of the proposed approach on two real-life in-house datasets further augmented to create a dual occupant setup, shows that the framework can correctly annotate a significant volume of unlabeled IMU data from both individuals with an accuracy of $\mathbf{82.59\%}$ ($\mathbf{\pm 17.94\%}$) and $\mathbf{98.32\%}$ ($\mathbf{\pm 3.68\%}$), respectively, for a workshop and a kitchen environment.

==> sections/motivation.tex <==
\section{Pilot Study}
\label{pilot}
Before designing the framework we first perform a set of pilot experiments, using the dataset mentioned above, to understand the opportunities and the challenges surrounding the problem statement. The details of the pilot experiments and the final lessons learned follow.
\subsection{Observations}
We start the pilot study by first looking into the un-augmented version of the datasets and identifying the user behavior while performing the activities. From Figure~\ref{fig:workshop_observations} and Figure~\ref{fig:kitchen_observations}, we can observe that most of the users tend to give occasional stops while performing physical activities. Indeed, this behavior heavily depends on the nature of the environment (workshop or kitchen) and the activities that are being performed. For example, in a workshop, we observe the stops are primarily given out of physical exertion, whereas for kitchen-based activities, the user may have to give intermediate stops due to the inherent nature of tasks like waiting for the food to get properly cooked or cleaning the chopping board. Interestingly, the diverse nature of these two environments is also highlighted in the average stop duration (see Figure~\ref{fig:stop_duration} and Figure~\ref{fig:stop_durations_kitchen}), which is significantly higher for kitchen based activities.

Focusing further on these stops and analyzing the changes in the input modalities, we observe that these opportunistic stops indeed create significant changes in the observed signatures. From Figure~\ref{fig:audio_change}, we observe that whenever a user stops, the signal changes significantly with occasional changes due to external noise. A similar analysis on the frequency domain characteristics of the augmented acoustic signatures (See Figure~\ref{fig:mixed_audio_change}) shows the frequency signatures change significantly once one activity stops, albeit the presence of external noise and presence of another source complicates the detection.

Concerning the IMU signatures (See Figure~\ref{fig:imu_change_pilot}), the analysis reveals a similar behavior, albeit with a slightly smaller window compared to the acoustic change. This is because when the user stops performing the activity, the acoustic signature drops immediately, while the IMU signatures still record the transition. For example, when a user resumes using a saw, the acoustic signature captures this instantly; however, the change starts a bit earlier for the IMU signature as the user may take the saw and prepare for resuming the activity.
\begin{figure}[]
	\captionsetup[subfigure]{}
	\begin{center}
		\subfloat[\label{fig:stop_counts}]{
			\includegraphics[width=0.48\linewidth,keepaspectratio]{figures/stop_counts.png}
		}
		\subfloat[\label{fig:stop_duration}]{
			\includegraphics[width=0.48\linewidth,keepaspectratio]{figures/stop_duration.png}
		}
	\end{center}
	\caption{Observations from the pilot experiment -- (a) Count of no. of stop intervals for users performing the two workshop activities, (b) Average stop duration.}
	\label{fig:workshop_observations}
\end{figure}
\begin{figure}[]
	\captionsetup[subfigure]{}
	\begin{center}
		\subfloat[\label{fig:stop_counts_kitchen}]{
			\includegraphics[width=0.48\linewidth,keepaspectratio]{figures/stop_counts_kitchen.png}
		}
		\subfloat[\label{fig:stop_durations_kitchen}]{
			\includegraphics[width=0.48\linewidth,keepaspectratio]{figures/stop_duration_kitchen.png}
		}
	\end{center}
	\caption{Observations from the pilot experiment -- (a) Count of no. of stop intervals for users performing the two kitchen activities, (b) Average stop duration. Here, users $\mathbf{U1}$ and $\mathbf{U2}$ perform chopping, whereas, users $\mathbf{U2}$, $\mathbf{U3}$, and $\mathbf{U4}$ perform the activity of cooking.}
	\label{fig:kitchen_observations}
\end{figure}
\begin{figure*}[]
	\captionsetup[subfigure]{}
	\begin{center}
		\subfloat[\label{fig:audio_change}]{
			\includegraphics[width=0.33\linewidth,keepaspectratio]{figures/pilot_audio_1.png}
		}
		\subfloat[\label{fig:mixed_audio_change}]{
			\includegraphics[width=0.33\linewidth,keepaspectratio]{figures/pilot_fft.png}
		}
		\subfloat[\label{fig:imu_change_pilot}]{
			\includegraphics[width=0.33\linewidth,keepaspectratio]{figures/imu_changes_pilot.png}
		}
	\end{center}
	\caption{Observations from the pilot experiment -- (a) Change in the acoustic context of a in single-user setting, (b) Change in single-sided amplitude spectrum of the environmental context when both activities vs. when only a single activity is getting performed and (c) Change in the IMU signatures of a user with respect to changes in activity patterns.}
\end{figure*}
\subsection{Lessons Learned}
Based on the aforementioned pilot study, we develop the following understanding regarding the opportunities and the subsequent challenges. Firstly, we understand that the users give occasional stops while performing any activity, and this provides us an opportunistic window to correctly annotate the IMU stream for the other user present in the smart environment. However, detecting these stops in an unsupervised manner is not straightforward. Interestingly, we observe that these stops are well reflected in both the IMU signatures and the global acoustic context, albeit sophisticated processing might be needed to differentiate between the relevant changes due to stops from the changes due to noise components. Most notably, we observe that the duration of the acoustic change due to a stop is slightly higher than the change in the IMU signature as the global audio does not change until the user resumes the activity; however, the IMU might change because of the intermediate transitions.
